ARENA: Asynchronous Reconfigurable Accelerator Ring to Enable Data-Centric Parallel Computing

The next generation HPC and data centers are likely to be reconfigurable and data-centric due to the trend of hardware specialization and the emergence of data-driven applications. In this paper, we propose ARENA -- an asynchronous reconfigurable accelerator ring architecture as a potential scenario on how the future HPC and data centers will be like. Despite using the coarse-grained reconfigurable arrays (CGRAs) as the substrate platform, our key contribution is not only the CGRA-cluster design itself, but also the ensemble of a new architecture and programming model that enables asynchronous tasking across a cluster of reconfigurable nodes, so as to bring specialized computation to the data rather than the reverse. We presume distributed data storage without asserting any prior knowledge on the data distribution. Hardware specialization occurs at runtime when a task finds the majority of data it requires are available at the present node. In other words, we dynamically generate specialized CGRA accelerators where the data reside. The asynchronous tasking for bringing computation to data is achieved by circulating the task token, which describes the data-flow graphs to be executed for a task, among the CGRA cluster connected by a fast ring network. Evaluations on a set of HPC and data-driven applications across different domains show that ARENA can provide better parallel scalability with reduced data movement (53.9%). Compared with contemporary compute-centric parallel models, ARENA can bring on average 4.37x speedup. The synthesized CGRAs and their task-dispatchers only occupy 2.93mm^2 chip area under 45nm process technology and can run at 800MHz with on average 759.8mW power consumption. ARENA also supports the concurrent execution of multi-applications, offering ideal architectural support for future high-performance parallel computing and data analytics systems.

==> sec-abstract.tex <==
%=========================================================================
% Abstract
%=========================================================================

\begin{abstract}
The next generation HPC and data centers are likely to be reconfigurable and data-centric due to the trend of hardware specialization and the emergence of data-driven applications. In this paper, we propose ARENA -- an asynchronous reconfigurable accelerator ring architecture as a potential solution on how the future HPC and data centers will be like. Despite using the coarse-grained reconfigurable arrays (CGRAs) as the substrate platform, our key contribution is not only the CGRA-cluster design itself, but the ensemble of a new architecture and programming model that enables asynchronous tasking across a cluster of reconfigurable nodes, so as to bring specialized computation to the data rather than the reverse. We presume distributed data storage without asserting any prior knowledge on the exact data distribution. Hardware specialization occurs at runtime when a task finds the majority of data it requires are available in the present node. In other words, we dynamically generate specialized CGRA accelerators where the data reside. The asynchronous tasking for bringing computation to data is achieved by circulating the task token, which describes the dataflow graphs to be executed for a task, among the CGRA cluster connected by a fast ring network. Evaluations on a set of HPC and data-driven applications across different domains show that ARENA can provide better parallel scalability with reduced data movement (53.9\%). Compared with contemporary compute-centric parallel models, ARENA can bring on average 4.37$\times$ speedup. The synthesized CGRAs and their task-dispatchers only occupy 2.93mm$^2$ chip area under 45nm process technology and can run at 800MHz with on average 759.8mW power consumption. ARENA also supports the concurrent execution of multi-applications, offering ideal architectural support for future HPC and high-performance data analytics systems.


%take only only 2.93mm$^2$ area and run at 800MHz with average 759.8mW power consumption. Moreover, ARENA's multiple CGRA accelerators can be dynamically and partially configured, which enables asynchronous execution and simultaneous acceleration of multi-user applications with trivial reconfiguration overhead.

%Evaluations on a set of representative HPC kernels and applications show that ARENA can bring 1.56X and 3.38X speedup over the baseline representing the contemporary compute-centric models with and without acceleration, respectively, and reduces data movement by 51.6\%. 


%Baseline: Computation-centric. Core is fixed, so computation capability is fixed. Data have to be moved to local to match the computation capability (threads, cores of the local). Our method is data-centric. Data is distributed among nodes and are fixed. Computation now is reconfigurable, so computation can be moved to data to match the granularity of the data. In this way, data movement can be reduced and computation utilization can be improved. 

%We take the first step towards filling this void through ARENA — an Asynchronous REcoNfigurable Accelerator ring for the next generation HPC clusters.

\end{abstract}



==> sec-casestudy.tex <==
%=========================================================================
% Casestudy
%=========================================================================

\section{Case Study}\label{sec:casestudy}
\sloppy
We present a case study to illustrate the features and impacts of the ARENA system architecture employed in an HPC cluster. We choose \textbf{breadth-first search} (BFS) kernel that solves the single source shortest path problem as our driving application kernel. The kernel traverses necessary vertices until the shortest paths from a source node to all the other nodes are found. In this case study, we represent a graph as an adjacency matrix that is distributed on an HPC cluster with a distributed memory system. Without loss of generality, we let each HPC node own $SIZE/NODES$ vertices (rows) of the entire graph (adjacency matrix of $SIZE$ x $SIZE$, $\infty$ indicates an edge while 0 indicates no connection).

\begin{figure}[!htb]
\begin{lstlisting}[basicstyle={\scriptsize\fontencoding{T1}\footnotesize\fontfamily{lmtt}\fontseries{c}\selectfont},escapechar=!]
int** local_M;
int num_visit;
...
int BFS_kernel(int vertex, int level) {
  for(int i=0; i<SIZE; ++i) {
    if(local_M[vertex][i] > level) {
      local_M[vertex][i] = level;
      visit_vertices[rank][num_visit] = i;
      num_visit += 1;
    }
  }
}
void run() {
  // Initialize local variables (e.g., local
  // partition of adjacency matrix: local_M)
  init();
  // Source vertex is launched on certain node
  if(local_start <= src and src < local_end) {
    num_visit = 0;
    visit_vertices[rank][num_visit] = src;
    num_visit += 1;
    level = 1;
  }
  while(1) {
    // Indicate #values will be broadcast
    Allgather(&num_visit, 1, num_all, 1);
    for(int i=0; i<NODES; ++i)
      if(num_all[i] > 0)
        // Broadcast the visited vertices
        Bcast(visit_vertices[i],num_all[i],i);
        
    for(int i=0; i<NODES; ++i)
      for(int j=0; j<num_all[i]; ++j)
        recv_q.push(visit_vertices[i][j]);
 
    num_visit = 0;
    if(recv_q.empty())
      break;
    while(recv_q.size()>0) {
      int v = recv_q.front();
      recv_q.pop();
      if(local_start <= v and v < local_end)
        BFS_kernel(v-local_bound, level);
      ++level;
    }
  }
}
\end{lstlisting}
\caption{A typical compute-centric BFS implementation.}
\label{fig:bfs_convention_impl}
\end{figure}

Conventional compute-centric BFS implementation requires considerable data communication and synchronization~\cite{bulucc2011parallel}. A typical implementation can be seen in Figure~\ref{fig:bfs_convention_impl}. Each HPC node only maintains the status (visited or not) of vertices it owns. Only the owner node of a vertice can identify whether it is newly visited or not. Thus, all the adjacencies of the vertices in the current frontier on a node need to be sent to their corresponding owner node, which incurs a set of all-to-all communications especially when each node is not aware of the global vertex distribution.

In contrast, ARENA enables an asynchronous data-centric execution model. Neither all-to-all data communication nor synchronization is needed. Task tokens are delivered via ARENA's ring topology and a task token will be picked by the node that contains the data range indicated by $TASK_{start}$ and $TASK_{end}$. Each HPC node then invokes the CGRA accelerator to perform the kernel execution. A typical data-centric implementation of BFS kernel is illustrated in Figure~\ref{fig:bfs_arena_impl}. \textit{ARENA\_spawn} can spawn a new task token, which will be dispatched by the current node itself or delivered to the next node on ARENA's ring. Once a task token is picked and executed by a node, multiple new tokens might be spawned. In this way, the entire graph will be traversed. We first evaluate the performance of BFS kernels in different execution models running on a CPU-only HPC cluster. Figure~\ref{fig:bfs_perf} shows that the data-centric execution model improves the performance with better scalability than the conventional compute-centric one.

\begin{figure}[htb]
	\centering
	\includegraphics[width=\cw]{graphs/evaluate_bfs_scale.pdf}
	\caption{Performance of BFS kernels running on different architectures.}
	\label{fig:bfs_perf}
\end{figure}

We also evaluate the ARENA with the hardware support of the dispatcher and CGRA. Our compiler toolchain can generate control signals of the ARENA task for different CGRAs. In addition, the compiler can lower the \textit{ARENA\_spawn} function as a $spawn$ operation supported by our CGRA's functional unit (four nodes in green color at the right most column as shown in Figure~\ref{fig:arena_node}).

CGRA can accelerates the execution of BFS by exacting the data parallelism and pipelining loop iterations. The 8x8 CGRA can be partitioned into four 2x8 CGRA groups, which enables different normalized speedups for BFS kernel supported by our compiler: 8.2X for a 2x8 CGRA, 16.4X for a 4x8 CGRA, and 21.8X for a 8x8 CGRA compared with an in-order execution without any acceleration (i.e., single cycle per operation). Note that the speedup of single 8x8 CGRA are less than the speedup of four 2x8 CGRAs (i.e., 21.8 $<$ 4 $\times$ 8.2). In conventional compute-centric model, entire 8x8 CGRA should be used to maximize the speedup of the level-synchronous BFS kernel (Figure~\ref{fig:bfs_convention_impl}). However, ARENA's asynchronous data-centric model efficiently utilizes the CGRA computing resources based on the required data range of the target task (discussed in Section~\ref{subsec:cgra}). To be specific, one group of 2x8 CGRA tiles are allocated to each data-centric BFS kernel (Figure~\ref{fig:bfs_arena_impl}). Since new tasks are spawned asynchronously at runtime, at most four groups can accelerate four BFS kernels simultaneously, which improves the overall speedup (as shown in Figure~\ref{fig:bfs_perf}) and the CGRA's area-efficiency. 

\todo[inline]{briefly mention DNA, GCN user cases.}

\todo[inline]{mention multi-user application scenario.}
